CompDiff enables fair and zero shot medical image generation across demographic intersections through compositional diffusion

Medical image generators trained on imbalanced data can fail at demographic intersections absent from training. We introduce CompDiff, which encodes age, sex and race separately and composes supervised demographic tokens alongside clinical text. Across chest radiographs and fundus images, CompDiff improves overall and subgroup fidelity relative to prompt conditioning (RoentGen-v2) and loss reweighting (FairDiffusion). It generalises in zero-shot generation to 16 chest X-ray intersections excluded from training, achieving the lowest mean FID-RadImageNet in every intersection. In a blinded reader study of these unseen intersections, two radiologists gave CompDiff the highest mean scores among generators for anatomical realism and agreement with the clinical impression, and selected its images most often as the most realistic. Pretraining with CompDiff images improved downstream classification, while CompDiff audit cohorts reduced estimation error on rare intersections. These findings support compositional demographic conditioning for extending medical image synthesis to underserved populations. Code: https://github.com/mahmoudibrahim98/CompDiff

==> main-labels.tex <==
% Generated from main.aux: label numbering of the sibling document, read when its .aux file is absent.
\newlabel{sec:intro}{{1}{2}{Introduction}{section.1}{}}
\newlabel{sec:related-work}{{1}{2}{Introduction}{section.1}{}}
\newlabel{subsec:rw-fair-medical}{{1}{2}{Introduction}{section.1}{}}
\newlabel{fig:problem}{{1}{3}{CompDiff: generating across demographic intersections to support learning and fairness auditing. \textbf {(a)} Uneven demographic coverage leaves some combinations of age, sex and race absent from training. \textbf {(b)} The Hierarchical Conditioner Network (HCN) composes supervised demographic tokens, which guide diffusion alongside separately encoded clinical text. Coverage and model diagrams are schematic. \textbf {(c)} Generation is assessed through a blinded radiologist study of intersections withheld from training and comparisons of overall and subgroup fidelity. The example plot shows overall chest X-ray Fr\'echet inception distance with RadImageNet features (FID-RN), with standard deviations across three training runs. \textbf {(d)} Synthetic training is evaluated for overall classification and for the weakest demographic groups. Diamonds show CompDiff's overall gains over RoentGen-v2 after training on synthetic images alone; bars show gains for the baseline's weakest groups after synthetic pretraining and fine-tuning on real images. Diamonds have pointwise 95\% Welch confidence intervals from four classifier runs per generator and corpus, averaging four corpora equally. Bars show medians across 48 configurations evaluated on both test datasets. \textbf {(e)} Synthetic cohorts audit a fixed classifier in two ways: reproducing evaluations on real data overall and improving the accuracy and precision of estimates for small subgroups. Upper points show absolute error relative to real-data evaluation. Below, real and CompDiff estimates for Asian women aged $\numResultsEO $--$\numResultsEP $ are compared with the dashed real reference; intervals are 95\% bootstrap confidence intervals from 1,000 resamples. AUROC denotes area under the receiver operating characteristic curve; panel (d) averages eight diagnostic labels. Grey, orange and green denote RoentGen-v2, FairDiffusion and CompDiff; blue denotes real data}{figure.caption.1}{}}
\newlabel{tab:methods-comparison}{{1}{4}{Conditioning and fairness mechanisms relevant to CompDiff. The table distinguishes the intervention and the task it supports; it does not report a matched performance comparison with every cited system. The fused demographic embedding and second text branch are controls from this study. The unstructured composer with a matched parameter count retains CompDiff's separate attribute encoders and supervised output tokens}{table.caption.2}{}}
\newlabel{fig:architecture}{{2}{5}{\textbf {CompDiff architecture and demographic conditioning.} \textbf {a,} RoentGen-v2 encodes clinical and demographic text together through CLIP's 77-token context. CompDiff encodes the clinical impression through CLIP and age, sex and race through the Hierarchical Conditioner Network (HCN). HCN supplies $\numMainFiguresI {}$ additional context tokens, concatenated with the text tokens before diffusion UNet cross-attention. \textbf {b,} HCN encodes age continuously and sex and race with separate categorical embeddings. Three dedicated multilayer perceptrons (MLPs) combine the attribute pairs; a composition MLP fuses their outputs into a shared demographic context. Each attribute embedding is concatenated with this context and projected to its own token. A Gaussian latent supplies only the composed token: it is sampled during training and set to its mean at inference. The four projected tokens each have 1,024 dimensions. Auxiliary heads supervise age, sex and race from their respective tokens and the joint demographic label from the composed token. Dashed arrows mark this training-only supervision; CE denotes cross-entropy}{figure.caption.3}{}}
\newlabel{sec:results}{{2}{6}{Results}{section.2}{}}
\newlabel{subsec:overall}{{2.1}{6}{Generation fidelity and alignment}{subsection.2.1}{}}
\newlabel{fig:overall}{{3}{7}{Overall generation quality across chest X-ray and fundus modalities. \textbf {a}--\textbf {d}, Metrics computed for both modalities, each panel showing a chest group and a fundus group: \textbf {a}, FID; \textbf {b}, FID-RadImageNet; \textbf {c}, MS-SSIM; \textbf {d}, mean AUROC. \textbf {e}--\textbf {h}, Agreement with the requested findings and demographic attributes for chest images: \textbf {e}, BioViL; \textbf {f}, sex accuracy; \textbf {g}, race accuracy; \textbf {h}, age RMSE. Each group contains the three methods (Baseline SD, FairDiffusion, CompDiff). A star and a green outline mark the best method within a group, and an upward arrow in a panel title indicates that higher is better and a downward arrow that lower is better; MS-SSIM carries neither, because neither tail is desirable and values are read against the defensible band $\numMainFiguresK {}$--$\numMainFiguresL {}$. Chest and Fundus bars are the mean over three independently trained runs per method, evaluated on the corresponding evaluation split, with error bars giving the standard deviation across those runs. Demographic and vision--language classifiers trained on chest images are out of domain on fundus images and are therefore reported for chest only}{figure.caption.4}{}}
\newlabel{tab:overall-pr}{{2}{7}{Distributional fidelity and coverage on the full chest X-ray test set with its natural demographic distribution, computed in RadImageNet ResNet-50 feature space with $k=10$ manifold neighbours. Higher is better for all four metrics. Precision~\cite {kynkaanniemi2019precision} and Density~\cite {naeem2020reliable} measure \emph {fidelity} (how often synthetic samples fall inside the real manifold), with Density a refinement of Precision that is less sensitive to outliers. Recall~\cite {kynkaanniemi2019precision} and Coverage~\cite {naeem2020reliable} measure \emph {diversity} (how much of the real manifold is reached by synthetic samples), with Coverage the replacement for Recall that is robust to mode collapse (uses manifold radii measured on real images rather than synthetic images, so it is not inflated by synthetic outliers)}{table.caption.8}{}}
\newlabel{fig:umap}{{4}{8}{Joint UMAP projection of chest X-ray RadImageNet features. One UMAP was fitted to pooled real and synthetic ResNet-\numMainFiguresM {} features, giving all panels shared axes. The same real cohort appears in warm grey beneath each generator's samples: RoentGen-v2 (Baseline SD, light grey), FairDiffusion (red) and CompDiff (green). CompDiff shows greater overlap with the cloud of real images. This projection is qualitative; Precision, Recall, Density and Coverage in Table~\ref {tab:overall-pr} quantify the distributions in the original feature space}{figure.caption.5}{}}
\newlabel{subsec:fairness}{{2.2}{9}{Subgroup generation quality}{subsection.2.2}{}}
\newlabel{subsec:zeroshot}{{2.3}{9}{Generation at unseen intersections}{subsection.2.3}{}}
\newlabel{fig:intersectional}{{5}{10}{Intersectional generation quality (lower is better). Left column (\textbf {a}, \textbf {c}, \textbf {e}, \textbf {g}): chest X-ray; right column (\textbf {b}, \textbf {d}, \textbf {f}, \textbf {h}): fundus. \textbf {a}, \textbf {b}, Overall distance and equity-scaled distance (ES-FID) across sex, race, age, and the full age $\times $ sex $\times $ race intersection (A$\times $S$\times $R), where the intersectional ES-FID uses every demographic cell as the subgroup list. \textbf {c}, \textbf {d}, By sex. \textbf {e}, \textbf {f}, By race. \textbf {g}, \textbf {h}, Per age bin. Each row groups three methods (Baseline SD, FairDiffusion, CompDiff), and a star marks the best method per row. The chest column reports FID-RadImageNet and the fundus column reports Inception FID, following the rationale for the feature backbone of Section~\ref {subsec:eval-synth}. Bars are means over three independently trained runs per method, with error bars giving the standard deviation across those runs. The fundus intersectional ES-FID is dominated by its dispersion term, because cell distances at the small fundus cell sizes are several times the overall distance; it is reported for completeness. The Hispanic row is omitted in panel \textbf {f} because the FairGenMed test set does not include Hispanic patients}{figure.caption.9}{}}
\newlabel{fig:zeroshot}{{6}{11}{Zero-shot generation across repeated training runs. Each method was trained three times on each of two holdouts, each withholding eight demographic intersections. FID-RadImageNet measures the distance between real and synthetic feature distributions within an intersection; lower values indicate closer agreement. \textbf {a,b}, Mean distance across the eight withheld cells for each trained model (open circles), with the mean across three models shown as a filled diamond. Runs are not paired by seed number. \textbf {c,d}, CompDiff minus comparator differences, averaged equally across cells and holdouts. Each panel shows one difference and its pointwise $\scLevel \%$ Welch--Satterthwaite confidence interval, with a separate zero reference and a common scale. Negative differences favour CompDiff. Each comparison uses twelve trained models; the experiment contains $\scModels $ models in total. Intervals describe variation across training, checkpoint selection and generation on the fixed test cohorts. Cell observations and means appear in Supplementary Figure~\ref {fig:zeroshot-cells}}{figure.caption.10}{}}
\newlabel{fig:qualitative_grid}{{7}{12}{Qualitative samples across tiers of subgroup rarity on both modalities. \textbf {Chest X-ray (MIMIC-CXR), top three rows}: \emph {Common} (\numMainFiguresU {}--\numMainFiguresV {} Male, White; $\numMainFiguresW {}\%$ of training), \emph {Rare} (\numMainFiguresX {}--\numMainFiguresY {} Female, Asian; $\numMainFiguresZ {}\%$ of training), and \emph {Zero-shot (withheld)} (\numMainFiguresAA {}+ Male, Asian; one of the eight intersections held out from training in the zero-shot protocol of Section~\ref {subsec:zeroshot-protocol}). \textbf {Fundus (FairGenMed), bottom two rows}: \emph {Common} (\numMainFiguresAB {}--\numMainFiguresAC {} Male, White) and \emph {Rare} (\numMainFiguresAD {}+ Male, Black). The two Common chest/fundus rows, the Rare chest row, and the Rare fundus row are sampled from generators trained on the natural demographic distribution; the Zero-shot chest row is sampled from the generators of Section~\ref {subsec:zeroshot-protocol}, trained with these intersections held out, so that row probes whether each generator can synthesise a demographic intersection it has never observed in training. Within each row, three samples with matched prompts are shown per method (Baseline SD, FairDiffusion, CompDiff); samples in the same column position across the three methods share the same clinical prompt, allowing visual comparison under the same clinical conditioning. The Zero-shot chest row prompts (all \numMainFiguresAE {}+ Male, Asian) are, left to right: a new large mass in the left upper lobe with rightward tracheal deviation concerning for malignancy; moderate cardiomegaly without pulmonary oedema or pleural effusion; and right basal atelectasis without pneumothorax}{figure.caption.11}{}}
\newlabel{subsec:reader-study}{{2.4}{13}{Radiologist assessment of unseen intersections}{subsection.2.4}{}}
\newlabel{tab:reader-study}{{3}{13}{Blinded radiologist assessment of chest X-ray sources on the zero-shot withheld intersections, by two board-certified radiologists ($\rsNInstances $ rater--set instances over $\rsNSets $ distinct sets, $\rsNRatings $ image ratings, across both withheld splits). Every rated image is of a demographic intersection absent from generator training. Realism is scored $1$--$5$ and prompt correspondence from $-2$ to $+2$ (mean $\pm $ SD; unreadable images excluded from realism, unreadable and N/A from correspondence). ``Most realistic'' is the per-set forced-choice win rate: the fraction of rated sets containing that source in which it was picked as the most realistic image. Real images are a hidden upper anchor present in a subset of sets}{table.caption.12}{}}
\newlabel{subsec:downstream}{{2.5}{13}{Downstream classification}{subsection.2.5}{}}
\newlabel{fig:downstream_combined}{{8}{14}{Downstream classifier performance when trained on synthetic data and evaluated on real test sets. \textbf {a}, \textbf {b}, AUC (higher is better) on chest X-ray (\textbf {a}) and fundus (\textbf {b}). \textbf {c}, \textbf {d}, Subgroup fairness (lower is better): underdiagnosis rate for chest (\textbf {c}) and equalised-odds difference for fundus (\textbf {d}). Each panel reports an overall result and separate summaries for sex, race and age and shows three methods (Baseline SD, FairDiffusion, CompDiff). Error bars are standard deviation across runs. The winning method per subgroup is outlined in dark slate and its label is bold. CompDiff is the winner on every chest X-ray (subgroup, metric) cell and on $\numMainFiguresAF {}/\numMainFiguresAG {}$ fundus cells}{figure.caption.13}{}}
\newlabel{fig:downstream-d3deep}{{9}{15}{Diagnostic utility of CompDiff images relative to RoentGen-v2. All panels use the same eight diagnostic labels. \textbf {(a)} AUROC$_8$ difference for classifiers trained on synthetic chest images alone. Diamonds show the contrast averaged equally across four fixed corpus regimes; bars are pointwise 95\% Welch confidence intervals based on four independent classifier runs per generator and regime, conditional on the corpora and real test cohorts. \textbf {(b)} Mean AUROC difference for each label across all 48 matched configurations with pretraining followed by fine-tuning. \textbf {(c)} Mean sensitivity difference at 90\% specificity over the same configurations. Sensitivity is read separately from each test ROC for this exploratory comparison; it does not represent a validated clinical threshold. Panels (b) and (c) are descriptive averages over configurations that share training data and test cohorts. All differences are CompDiff minus RoentGen-v2; positive values favour CompDiff. Colours identify the test dataset. The same trained models are evaluated on both datasets}{figure.caption.16}{}}
\newlabel{tab:recipes}{{4}{16}{Downstream classifier training recipes. Each recipe is evaluated for both CompDiff and the RoentGen-v2 baseline. The natural synthetic corpora match the demographic distribution of the MIMIC-CXR training split, while the balanced corpus is expanded to approximately uniform coverage of $(\text {age}, \text {sex}, \text {race})$ cells. The pretrain $\rightarrow $ real fine-tune family is additionally swept over six fractions of real data (1\%, 10\%, 30\%, 50\%, 70\%, 100\%), giving 48 matched configurations per evaluation dataset. Balanced-corpus counts are $\dsBalancedRG $ for RoentGen-v2 and $\dsBalancedCD $ for CompDiff}{table.caption.15}{}}
\newlabel{fig:pergroup-disparity}{{10}{17}{Subgroup gains across the complete downstream training sweep. \textbf {(a)} CompDiff minus RoentGen-v2 AUROC$_8$ for each sex, race and age group, shown separately for MIMIC-CXR and CheXpert. \textbf {(b)} Gain for the subgroup with the lowest RoentGen-v2 AUROC within each demographic attribute in each configuration, retaining its identity under CompDiff. Hollow circles show the 48 configuration differences; filled diamonds and thick bars show medians and interquartile ranges. These ranges describe variation across configurations, not confidence intervals. Counts in (b) give configurations with a positive gain. Every subgroup score averages the same eight labels, each with at least one positive and one negative image. Configurations share training data and test cohorts. Sample sizes and uncertainty checks for sparse groups are in Supplementary Tables~\ref {tab:downstream-groups} and~\ref {tab:downstream-uncertainty}}{figure.caption.18}{}}
\newlabel{subsec:eval-instrument}{{2.6}{18}{Synthetic cohorts for fairness auditing}{subsection.2.6}{}}
\newlabel{fig:audit-instrument}{{11}{19}{Agreement between synthetic and real test cohorts when auditing a fixed DenseNet-\numMainFiguresAP {} trained on real data. Each synthetic cohort matches the real test split in size and demographic distribution. Bars show absolute differences from the real test result; lower values indicate closer agreement. \textbf {a,} Overall errors for AUROC$_8$, AUROC$_{\numMainFiguresAQ {}}$ and underdiagnosis rate. \textbf {b,} Mean and largest absolute AUROC errors across marginal sex, race and age groups. \textbf {c,} Mean absolute AUROC error within each attribute and attribute pair. Colours identify the generator. A star marks the lowest observed error in each comparison, selected before rounding. All comparisons use a single fixed classifier}{figure.caption.19}{}}
\newlabel{fig:per-cell-calibration}{{12}{20}{Accuracy and precision of classifier evaluation on rare demographic intersections. A single DenseNet-\numMainFiguresAR {} trained on real data is evaluated using macro AUROC over \numMainFiguresAS {} labels. The independent real reference split is excluded from training and model selection. Each synthetic cohort matches its demographic distribution and cell sizes; the small real test cohort contains fewer images. \textbf {a,} Mean absolute difference from the reference AUROC across three rarity tiers of \numMainFiguresAV {}, \numMainFiguresAW {} and \numMainFiguresAX {} cells, ordered by reference cohort size. Grouped bars show the four estimators, with a star marking the lowest observed error in each tier. Lower error indicates greater accuracy relative to the reference. \textbf {b,} Mean \numMainFiguresAU {}\% confidence-interval width on the \numMainFiguresBA {} rarest cells. A star identifies the narrowest mean interval among all five cohorts, including the real reference. Narrower intervals indicate greater precision. \textbf {c,} AUROC estimates and \numMainFiguresAY {}\% bootstrap intervals for each of those cells, with the real reference marked by a plus. The displayed $n$ is the reference cell size. Intervals use \numMainFiguresAT {} bootstrap iterations. The same nine cells contribute to panels b and c. These are estimates for one classifier; panels a and b do not quantify variation across classifier training runs}{figure.caption.20}{}}
\newlabel{tab:ablations}{{5}{21}{Ablations, grouped by design question and ordered by effect size. All values are validation metrics at each run's own selected checkpoint, chosen by the rule used throughout this paper (Eq.~\ref {eq:ckpt-rule}: lowest validation FID among checkpoints meeting the controllability floors). Where a run has no eligible checkpoint we report its checkpoint with the lowest age RMSE, since in those runs the age floor is unreachable over the entire trajectory and so disqualifies every checkpoint. Rows marked $\ddagger $ were measured under the configuration in which age is conditioned through the text prompt and only sex and race pass through the conditioner; they are comparable among themselves and to the $\ddagger $ reference row. \emph {Floors} states whether the reported checkpoint meets the floors, and in each ablated row the value that decides its verdict is set in bold. FID-RN abbreviates FID-RadImageNet; AUROC is the XRV disease classifier AUROC on the synthetic images (prompt alignment, Section~\ref {subsec:eval-synth}), not a downstream classifier}{table.caption.23}{}}
\newlabel{subsec:ablations}{{2.7}{21}{Conditioning interface ablations}{subsection.2.7}{}}
\newlabel{sec:discussion}{{3}{22}{Discussion}{section.3}{}}
\newlabel{sec:methods}{{4}{24}{Methods}{section.4}{}}
\newlabel{sec:experiments}{{4}{24}{Methods}{section.4}{}}
\newlabel{subsec:datasets}{{4.1}{24}{Study design, datasets and ethics}{subsection.4.1}{}}
\newlabel{subsec:ethics}{{4.1}{24}{Study design, datasets and ethics}{subsection.4.1}{}}
\newlabel{subsec:objective}{{4.2}{25}{CompDiff architecture and objective}{subsection.4.2}{}}
\newlabel{app:implementation}{{4.2}{25}{CompDiff architecture and objective}{subsection.4.2}{}}
\newlabel{eq:loss}{{6}{26}{Training objective}{equation.6}{}}
\newlabel{eq:aux}{{8}{26}{Training objective}{equation.8}{}}
\newlabel{subsec:gen-training}{{4.3}{26}{Training, sampling and checkpoint selection}{subsection.4.3}{}}
\newlabel{subsec:gen-sampling}{{4.3}{26}{Training, sampling and checkpoint selection}{subsection.4.3}{}}
\newlabel{subsec:checkpoint-schedule}{{4.3}{26}{Training, sampling and checkpoint selection}{subsection.4.3}{}}
\newlabel{app:checkpoint-selection}{{4.3}{26}{Training, sampling and checkpoint selection}{subsection.4.3}{}}
\newlabel{eq:ckpt-rule}{{9}{27}{Training, sampling and checkpoint selection}{equation.9}{}}
\newlabel{subsec:eval-synth}{{4.4}{27}{Generation quality and unseen-intersection evaluation}{subsection.4.4}{}}
\newlabel{app:manifold-metrics}{{4.4}{27}{Generation quality and unseen-intersection evaluation}{subsection.4.4}{}}
\newlabel{subsec:zeroshot-protocol}{{4.4}{27}{Generation quality and unseen-intersection evaluation}{subsection.4.4}{}}
\newlabel{tab:metrics-summary}{{6}{28}{Summary of all metrics of generation quality used in this paper, grouped by measurement role; procedures are given in Section~\ref {subsec:eval-synth}. An upward arrow in the direction column indicates that higher values are better and a downward arrow that lower values are better. For MS-SSIM neither tail is desirable and we report whether the value falls inside the reference range $0.25$--$0.75$~\cite {moroianu2025improvingperformancerobustnessfairness}. Family (E) (ES-FID) is the extension for subgroup fairness used in Section~\ref {subsec:fairness}}{table.caption.30}{}}
\newlabel{subsec:reader-protocol}{{4.5}{30}{Radiologist reader study}{subsection.4.5}{}}
\newlabel{subsec:downstream-recipes}{{4.6}{30}{Downstream training and classifier auditing}{subsection.4.6}{}}
\newlabel{subsec:eval-protocol}{{4.6}{30}{Downstream training and classifier auditing}{subsection.4.6}{}}
\newlabel{subsec:composer-control}{{4.7}{31}{Conditioning and composer ablations}{subsection.4.7}{}}
\newlabel{subsec:clip-protocol}{{4.7}{32}{Supplementary analysis of demographic text}{section*.36}{}}
\newlabel{subsec:robustness-protocol}{{4.8}{32}{Fidelity robustness and sampling controls}{subsection.4.8}{}}
\newlabel{subsec:statistics}{{4.9}{33}{Statistical analysis and reporting}{subsection.4.9}{}}
\newlabel{eq:seed-contrast}{{11}{33}{Replication and comparisons across trained models}{equation.11}{}}
\newlabel{app:reader-stats}{{4.9}{34}{Reader ratings and preferences}{section*.38}{}}
\newlabel{eq:reader-lmm}{{12}{34}{Reader ratings and preferences}{equation.12}{}}

